E-Commerce Dispute Resolution Prediction

E-Commerce marketplaces support millions of daily transactions, and some disagreements between buyers and sellers are unavoidable. Resolving disputes in an accurate, fast, and fair manner is of great importance for maintaining a trustworthy platform. Simple cases can be automated, but intricate cases are not sufficiently addressed by hard-coded rules, and therefore most disputes are currently resolved by people. In this work we take a first step towards automatically assisting human agents in dispute resolution at scale. We construct a large dataset of disputes from the eBay online marketplace, and identify several interesting behavioral and linguistic patterns. We then train classifiers to predict dispute outcomes with high accuracy. We explore the model and the dataset, reporting interesting correlations, important features, and insights.

==> Figures/removed_text.tex <==
\remove{
\begin{table}[t]
\caption{Information gain of different features in the XGBoost model}
\label{xgboost_gains_table}
\begin{tabular}{|l|l|}
\hline
\textbf{Feature}                         & \textbf{Information Gain} \\ \hline
First escalating party                        & 117.555124                \\ \hline
Recent escalating party                         & 34.913347                 \\ \hline
Seller Response Yes/No                           & 32.486752                 \\ \hline
seller\_data\_user\_sts\_code            & 22.559289                 \\ \hline
seller\_data\_flagsex8\_3                & 21.589365                 \\ \hline
seller\_data\_user\_site\_id             & 20.087752                 \\ \hline
seller\_data\_flagsex9\_4                & 19.009521                 \\ \hline
SLR\_PREESC\_RSPNS\_YN                   & 13.038982                 \\ \hline
CLAIM\_TYPE                              & 12.737678                 \\ \hline
seller\_data\_user\_cntry\_id            & 11.856084                 \\ \hline
seller\_data\_top\_rated\_seller\_us\_yn & 10.234963                 \\ \hline
RTRN\_ESC\_YN\_IND                       & 8.914927                  \\ \hline
seller\_data\_ebx\_cs\_frc\_out\_yn\_id  & 8.350122                  \\ \hline
FINAL\_CLAIM\_TYPE                       & 8.166833                  \\ \hline
seller\_data\_last\_modfd                & 7.788413                  \\ \hline
buyer\_data\_user\_cntry\_id             & 7.768437                  \\ \hline
B2C\_C2C\_FLAG                           & 7.527530                  \\ \hline
buyer\_data\_flagsex2\_6                 & 6.448836                  \\ \hline
buyer\_data\_flagsex6\_7                 & 6.064697                  \\ \hline
\end{tabular}
\end{table}
}



\remove{
\begin{table}[t]
\caption{Information gain of different features in the XGBoost model}
\label{xgboost_gains_table}
\begin{tabular}{|l|l|}
\hline
\textbf{Feature}                         & \textbf{Information Gain} \\ \hline
FIRST\_ESC\_PARTY                        & 74.62364879916608         \\ \hline
RCNT\_ESC\_PARTY                         & 52.98509223446398         \\ \hline
SLR\_RSPNS\_YN                           & 24.772387485078223        \\ \hline
SLR\_PREESC\_RSPNS\_YN                   & 24.08417914395161         \\ \hline
seller\_data\_user\_site\_id             & 15.418236935354642        \\ \hline
seller\_data\_flagsex8\_3                & 15.10246659367649         \\ \hline
seller\_data\_flagsex9\_4                & 14.910555263697553        \\ \hline
CLAIM\_TYPE                              & 13.2912335711715          \\ \hline
seller\_data\_top\_rated\_seller\_us\_yn & 12.703958551561202        \\ \hline
\end{tabular}
\end{table}


}


==> Figures/removed_text_6.tex <==
\remove{
FIRST_ESC_PARTY                              119.654988
SLR_RSPNS_YN                                  39.985860
RCNT_ESC_PARTY                                26.324478
seller_data_flagsex8_13                       21.344336
CLAIM_TYPE                                    17.128960
seller_data_flagsex9_16                       16.024928
seller_data_user_site_id                      13.303492
seller_data_flagsex2_5                        12.709154
seller_data_dw_users_info_upd_date            11.848819
seller_data_user_cntry_id                     11.776476
seller_data_user_sts_code                     11.186821
seller_data_top_rated_seller_us_yn            10.320796
SLR_PREESC_RSPNS_YN                            7.837516
buyer_data_flagsex11_23                        6.947342
seller_data_flagsex7_3                         6.869537
RTRN_YN_IND                                    6.786455
seller_data_last_modfd                         6.493108
buyer_data_user_cntry_id                       6.455081
seller_data_flagsex11_11                       6.270448
FAST_TEXT_PREDICTION                           6.099392
B2C_C2C_FLAG                                   6.060306
}
\remove{
\begin{table}[t]
\caption{Information gain of different features in the XGBoost model}
\label{xgboost_gains_table}
\begin{tabular}{|l|l|}
\hline
\textbf{Feature}                         & \textbf{Information Gain} \\ \hline
First escalating party                        & 117.555124                \\ \hline
Recent escalating party                         & 34.913347                 \\ \hline
Seller Response Yes/No                           & 32.486752                 \\ \hline
Seller account status            & 22.559289                 \\ \hline
seller\_data\_flagsex8\_3                & 21.589365                 \\ \hline
Seller site ID                           & 20.087752                 \\ \hline
seller\_data\_flagsex9\_4                & 19.009521                 \\ \hline
Seller Pre-escalation Response Yes/No    & 13.038982                 \\ \hline
Claim Type                              & 12.737678                 \\ \hline
Seller Country                          & 11.856084                 \\ \hline
Top Rated Seller & 10.234963                 \\ \hline
Return Request                       & 8.914927                  \\ \hline
seller\_data\_ebx\_cs\_frc\_out\_yn\_id  & 8.350122                  \\ \hline
Final Claim Type                       & 8.166833                  \\ \hline
seller\_data\_last\_modfd                & 7.788413                  \\ \hline
Buyer Country             & 7.768437                  \\ \hline
Seller Type                           & 7.527530                  \\ \hline
\end{tabular}
\end{table}
}
%The only content of the claim is found in the claim type feature, which indicates whether the claim is INR or SNAD. \mnote{We should test whether this is still true while using the textual features}

